A Bayesian Approach to Recurrence in Neural Networks

We begin by reiterating that common neural network activation functions have simple Bayesian origins. In this spirit, we go on to show that Bayes's theorem also implies a simple recurrence relation; this leads to a Bayesian recurrent unit with a prescribed feedback formulation. We show that introduction of a context indicator leads to a variable feedback that is similar to the forget mechanism in conventional recurrent units. A similar approach leads to a probabilistic input gate. The Bayesian formulation leads naturally to the two pass algorithm of the Kalman smoother or forward-backward algorithm, meaning that inference naturally depends upon future inputs as well as past ones. Experiments on speech recognition confirm that the resulting architecture can perform as well as a bidirectional recurrent network with the same number of parameters as a unidirectional one. Further, when configured explicitly bidirectionally, the architecture can exceed the performance of a conventional bidirectional recurrence.

==> forget.tex <==
in place of equation
\ref{eq:FeatProb},
\begin{align}
  \hid_{t,i}
  &=
    \CondPr{\feat_{t,i}}{\OBS_{t},\HID_{t-1}} \\
  &=
    \sum_{\cvar_{t}}
    \CondPr{\feat_{t,i}}{\cvar_{t},\OBS_{t},\HID_{t-1}}
    \CondPr{\cvar_{t}}{\OBS_{t},\HID_{t-1}} \\
  &=
    \sum_{\cvar_{t}}
    \frac{%
    \CondLi{\Obs_t,\Hid_{t-1}}{\feat_{t,i},\cvar_{t},\OBS_{t-1},\HID_{t-2}}
    \CondPr{\feat_{t,i}}{\cvar_{t},\OBS_{t-1},\HID_{t-2}}
    }{\sum_{\feat_{t,i}}
    \CondLi{\Obs_t,\Hid_{t-1}}{\feat_{t,i},\cvar_{t},\OBS_{t-1},\HID_{t-2}}
    \CondPr{\feat_{t,i}}{\cvar_{t},\OBS_{t-1},\HID_{t-2}}
    }
    \CondPr{\cvar_{t}}{\OBS_{t},\HID_{t-1}} \\
  &= \frac{1}{1+
    \dfrac
    {\CondLi{\Obs_t,\Hid_{t-1}}{\bar\feat_{t,i}}}
    {\CondLi{\Obs_t,\Hid_{t-1}}{\feat_{t,i}}}
    \cdot\dfrac{
      \CondPr{\bar\feat_{t,i}}{\OBS_{t-1},\HID_{t-2}}
    }{
      \CondPr{\feat_{t,i}}{\OBS_{t-1},\HID_{t-2}}
    }
  },
\end{align}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% TeX-PDF-mode: t
%%% End:


==> gates.tex <==
\section{Gates}

Say we want a gate (or anything) to depend on the previous outputs.  The gate
is just the probability of a state variable, call it $\sigma$.  First state
that $\sigma$ depends upon the features:
\begin{equation}
  \CondPr{\sigma_{t}}{\OBS_{t}}
  =
  \sum_{\Feat_{t-1}}
  \CondPr{\sigma_{t}}{\Feat_{t-1},\OBS_{t}}
  \CondPr{\Feat_{t-1}}{\OBS_{t}}.
\end{equation}
If there is just one feature, we can write
\begin{equation}
  \CondPr{\sigma_{t}}{\OBS_{t}}
  =
  \CondPr{\sigma_{t}}{\feat_{t-1},\OBS_{t}}\hid_{t-1} +
  \CondPr{\sigma_{t}}{\bar\feat_{t-1},\OBS_{t}}(1-\hid_{t-1}).
\end{equation}
In the case of two features,
\begin{multline}
  \CondPr{\sigma_{t}}{\OBS_{t}}
  = \\
  \begin{split}
    & \CondPr{\sigma_{t}}{\feat_{1,t-1},\feat_{2,t-1},\OBS_{t}}
    \hid_{1,t-1}\hid_{2,t-1} +
    \CondPr{\sigma_{t}}{\bar\feat_{1,t-1},\feat_{2,t-1},\OBS_{t}}
    (1-\hid_{1,t-1})\hid_{2,t-1} + \\
    & \CondPr{\sigma_{t}}{\feat_{1,t-1},\bar\feat_{2,t-1},\OBS_{t}}
    \hid_{1,t-1}(1-\hid_{2,t-1}) +
    \CondPr{\sigma_{t}}{\bar\feat_{1,t-1},\bar\feat_{2,t-1},\OBS_{t}}
    (1-\hid_{1,t-1})(1-\hid_{2,t-1}).
  \end{split}
\end{multline}
In each case, it may be possible to attach a meaning to
$\CondPr{\sigma_{t}}{\feat_{t-1},\OBS_{t}}$; this was certainly true for the
probabilistic forget.  However, in general, this should be learned.  Further,
if a sigmoid is used, the required function is
$-\logit[\CondPr{\sigma_{t}}{\OBS_{t}}]$, which is rather complicated.  So we
arrive at the approximation
\begin{equation}
  -\logit[\CondPr{\sigma_{t}}{\OBS_{t}}] \approx
  \weight_\hid^\T\Hid_{t-1} + \bias_\hid,
\end{equation}
being a truncated Taylor series.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% TeX-PDF-mode: t
%%% End:


==> relevance.tex <==
\section{Relevance}

\subsection{Rationale}

Say there are some observations that are not relevant to the estimation of the
features.  Say there is a binary state variable, $\rvar$, where $\rvar=1$
indicates the input being relevant and $\rvar=0$ indicates that it is not
relevant.  We can assign a probability,
$\rlvn_t=\CondPr{\rvar_t=1}{\OBS_{t}}$.
In the following, we discuss some ways to handle this.

\subsection{Marginalise the output}

For a given feature, $\feat_i$,
\begin{align}
  \hid_{t,i}
  &= \CondPr{\feat_i}{\OBS_{t}} \\
  &= \sum_{\rvar_t}
    \CondPr{\feat_i}{\OBS_{t},\rvar_{t,i}}\CondLi{\rvar_{t,i}}{\OBS_t}\\
  &= (1-\rlvn_{t,i})\CondPr{\feat_i}{\OBS_{t-1}}
    + \rlvn_{t,i}\CondPr{\feat_i}{\OBS_{t}}\\
  &= (1-\rlvn_{t,i})\hid_{t-1,i} + \rlvn_{t,i}\CondPr{\feat_i}{\OBS_{t}}
\end{align}
This, again, correlates to the update function in GRU:
\begin{equation}
  h_t = (1 - z_t) n_t + z_t h_{(t-1)},
\end{equation}
where $n_t$ is defined as equation \ref{eq:gru} and $z_t$ is the update gate
computed as
\begin{equation}
  z_t = \sigma(\Weight_{iz} x_t + b_{iz} + \Weight_{hz} h_{(t-1)} + b_{hz})
\end{equation}

\subsection{Marginalise the input}

We should not expect the feature classifier to be able to make a decision.
With no prior information, this is represented by $\hid_{t,i}=0.5$; with prior
information we should just retain the prior, so
\begin{align}
  \frac
  {\CondLi{\Obs_t}{\bar\feat_i}}
  {\CondLi{\Obs_t}{\feat_i}}
  & = 1, \\
  \CondLi{\Obs_t}{\bar\feat_i} &=
  \CondLi{\Obs_t}{\feat_i} = C.
\end{align}

As before, we can then marginalise over $\rvar$:
\begin{align}
  \CondLi{\Obs_t}{\feat_{t,i},\rlvn_{t,i}}
  &= \sum_{\cvar_t}
    \CondLi{\Obs_t}{\rvar_{t,i},\feat_{t,i}}
    \CondLi{\rvar_{t,i}}{\feat_{t,i}} \\
  &= \rlvn_{t,i}\CondLi{\Obs_t}{\feat_{t,i}}
    + (1-\rlvn_{t,i})C.
\end{align}
The ratio is then
\begin{equation}
  \frac
  {\CondLi{\Obs_t}{\bar\feat_i,\rlvn_{t,i}}}
  {\CondLi{\Obs_t}{\feat_i,\rlvn_{t,i}}}
  =
  \frac{
    \rlvn_{t,i}\CondLi{\Obs_t}{\bar\feat_i} +
    (1-\rlvn_{t,i})C
  }{
    \rlvn_{t,i}\CondLi{\Obs_t}{\feat_i} +
    (1-\rlvn_{t,i})C
  }.
\end{equation}
It's intuitively reasonable, but tricky to implement.


\subsection{Variance scaling}

An alternative and much simpler approach would be to scale the variance.  If we
begin with the definition of the weights and bias from equations
\eqref{eq:TwoClassWeight} and \eqref{eq:TwoClassBias}, and ignore the priors in
the bias, it is clear that the scaling $\Weight$ and $\bias$ is equivalent to
scaling the precision, $\Covariance^{-1}$.  As the precision tends to zero, the
variance tends to infinity, reducing the discriminative ability of the
classifier.  So, we can imagine some canonical precision,
$\Tilde\Covariance^{-1}$, and the precision used in the actual neuron to be
function of it:
\begin{equation}
  \Covariance^{-1} = \rlvn\Tilde\Covariance^{-1},
\end{equation}
so, equation \ref{eq:TwoClass} becomes
\begin{equation}
  \CondPr{\class_1}{\Scalar} =
  \frac{1}{
    1+
    \exp\left(-\rlvn(\Weight^\T\Scalar + \bias\right))
  }.
\end{equation}
In the Boltzmann case this is equivalent to increasing the temperature; a
higher temperature implies less well defined probabilities.
\begin{figure}[htb]
  \centering
  \input{tikz-vsu}
  \caption{A variance scaled unit.}
  \label{fig:VSU}
\end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% TeX-PDF-mode: t
%%% End:

